InfoDeepSeek: Benchmarking Agentic Information Seeking for Retrieval-Augmented Generation

Retrieval-Augmented Generation (RAG) enhances large language models (LLMs) by grounding responses with retrieved information. As an emerging paradigm, Agentic RAG further enhances this process by introducing autonomous LLM agents into the information seeking process. However, existing benchmarks fall short in evaluating such systems, as they are confined to a static retrieval environment with a fixed, limited corpus} and simple queries that fail to elicit agentic behavior. Moreover, their evaluation protocols assess information seeking effectiveness by pre-defined gold sets of documents, making them unsuitable for the open-ended and dynamic nature of real-world web environments. To bridge this gap, we present InfoDeepSeek, a new benchmark with challenging questions designed for assessing agentic information seeking in real-world, dynamic web environments. We propose a systematic methodology for constructing challenging queries satisfying the criteria of determinacy, difficulty, and diversity. Based on this, we develop the first evaluation framework tailored to dynamic agentic information seeking, including fine-grained metrics about the accuracy, utility, and compactness of information seeking outcomes. Through extensive experiments across LLMs, search engines, and question types, InfoDeepSeek reveals nuanced agent behaviors and offers actionable insights for future research.

==> backup.tex <==
In recent years, large language models (LLMs) have demonstrated remarkable capabilities in various domains~\cite{lin2025can,hadi2023survey,wang2024survey,zhao2023survey,kasneci2023chatgpt,thirunavukarasu2023large,wei2022emergent}. However, they still suffer from factual hallucination~\cite{huang2025survey,martino2023knowledge}, outdated knowledge~\cite{he2022rethinking}, and insufficient domain expertise~\cite{shen2023chatgpt}. To mitigate this, Retrieval-Augmented Generation (RAG)~\cite{fan2024survey,gao2023retrieval,zhao2024retrieval} has emerged as a promising solution, enabling LLMs to produce more accurate and up-to-date responses with real-time information retrieval. Despite its promise, traditional RAG systems rely on static workflows, making them ill-suited for complex user queries or dynamic and noisy real-world search environments~\cite{singh2025agentic}. Recently, Agentic RAG~\cite{singh2025agentic,schneider2025collex,ravuru2024agentic,he2025pasa} addresses these shortcomings by incorporating LLM agents into the retrieval process. These agents are capable of dynamic decision-making,  iterative refinement, and workflow optimization, enabling more in-depth, robust, and flexible information-seeking\ljh{give a footnote, stating that information seeking in this paper refers to the complex/multi-turn information retrieval from various data sources balabala.} behaviors required for challenging and realistic tasks. 

\ljh{feels like information seeking refers to both stages of retrieval and augmentataion. searching collecting filtering and ranking}

\ljh{we should emphasize more on 'information seeking' instead of using terms retrieval}

\ljh{feels like we are benchmarking agentic rag instead of agentic information seeking}

\ljh{agentic rag的核心差异在于复杂信息查询（回答llm其实大差不差），但如今benchmark都难以准确评估agentic rag中的information seeking能力。具体两方面，数据库不行（static environment with fixed and limited data sources）,查询问题不行（不够复杂不够难）}

Agentic RAG methods have begun to see practical applications\ljh{begin to see xxx is somehow weired to me, maybe change the phrase} -- for example, OpenAI~\cite{openai_dr}, Gemini~\cite{gemini_dr}, and Perplexity~\cite{Perplexity_dr} have supported Deep Research that enables agents to perform iterative information seeking in real-world web environments. However,  the development of corresponding evaluation benchmarks has lagged significantly behind, posing substantial challenges to comprehensively assessing the capabilities of such systems. First\ljh{there is no 'second', suggest remove first}, most existing RAG benchmarks predominantly rely on retrieval from a static database~\cite{yang2024crag,chen2024rgb,lyu2401crud,tang2024multihop}, which fail to capture the dynamic and ever-changing nature of the real-world web environment, \eg, content updates, URL decay, and fluctuations in search engine results.\ljh{the content volume is also a difference, static database can always be small for agentic rag compared with the Internet} As a result, these benchmarks do not align well with the complexities that Agentic RAG systems must handle in deployment. Moreover, many questions in current benchmarks are not difficult enough, often answerable by LLMs with internal knowledge or a single retrieval step~\cite{vu2023freshllms,kwiatkowski2019NQ,tang2024multihop}. This limits the need for agentic behaviors such as planning and multi-turn search -- core components of Agentic RAG that remain under-assessed.

In real web environments, agentic retrieval \ljh{information seeking} often involves iterative exploration that generates evolving, redundant, and noisy information~\cite{wei2025browsecomp,pan2023kwaiagents}.  As a result, evaluating the quality of information that agents find and extract becomes critical. However, ground-truth documents cannot be pre-defined in such settings, rendering traditional metrics for retrieval quality, such as NDCG~\cite{yang2024crag}, inapplicable. Consequently, there is a growing need for a new evaluation paradigm that can assess the retrieval quality of Agentic RAG systems in open, dynamic environments.

To address the above limitations, we propose InfoDeepSeek, a novel benchmark tailored for agentic information-seeking tasks under real-world web environments. First, we introduce a set of criteria and a systematic methodology for constructing challenging queries aimed at evaluating agentic information seeking, and manually curate and validate 200 high-quality questions, each carefully designed to exhibit the following properties:
\begin{itemize}
    \item \textbf{Determinacy}: Each question has a clear, unique, and temporally stable answer.
    \item \textbf{Difficulty}: The questions are intentionally challenging for LLM, even with single-turn online search, thereby necessitating multi-turn agentic information seeking.
    \item \textbf{Diversity}: The challenging questions cover various domains, predominant languages, and attributes, including multi-hop, long tail, emerging facts, time sensitivity, distracting information, and false premises.
\end{itemize}

Building on this, we develop an agentic information-seeking system\ljh{is this our contribution?} that integrates multiple search and browsing tools, allowing agents to perform multi-turn search and planning in live web environments. Facing such a noisy and dynamic environment, we propose a set of fine-grained evaluation metrics and protocols to assess retrieval quality\ljh{assess the quality of information seeking results} dynamically. Our evaluation metrics include answer accuracy, retrieval accuracy, information compactness, and effective evidence utilization, offering a comprehensive view of the agent's information-seeking and extracting ability. We further conduct empirical evaluations across multiple dimensions, including different LLMs, search engines, and question types, revealing agents' behaviors under complex and dynamic environments. Our key contributions are as follows:
\begin{itemize}
    \item We introduce a set of criteria and a systematic methodology for constructing challenging queries and present a new benchmark\ljh{InfoDeepSeek} for evaluating agentic RAG in real-world settings. \ljh{We believe these principles and methodologies are transferable and can benefit the research community of benchmarking AI agents for RAG. (benefit xxx, I am not sure)}
    \item We propose a general Agentic RAG framework coupled with fine-grained evaluation metrics and protocols that assess the retrieval quality of agents in dynamic open environments.
    \item We provide a comprehensive comparison of agents under different LLMs, search engines, and question types, identifying their limitations and outlining directions for future research.

\end{itemize}


